Factorized-FL: Agnostic Personalized Federated Learning with Kernel Factorization & Similarity Matching

In real-world federated learning scenarios, participants could have their own personalized labels which are incompatible with those from other clients, due to using different label permutations or tackling completely different tasks or domains. However, most existing FL approaches cannot effectively tackle such extremely heterogeneous scenarios since they often assume that (1) all participants use a synchronized set of labels, and (2) they train on the same task from the same domain. In this work, to tackle these challenges, we introduce Factorized-FL, which allows to effectively tackle label- and task-heterogeneous federated learning settings by factorizing the model parameters into a pair of vectors, where one captures the common knowledge across different labels and tasks and the other captures knowledge specific to the task each local model tackles. Moreover, based on the distance in the client-specific vector space, Factorized-FL performs selective aggregation scheme to utilize only the knowledge from the relevant participants for each client. We extensively validate our method on both label- and domain-heterogeneous settings, on which it outperforms the state-of-the-art personalized federated learning methods.

==> figures/fig_analysis.tex <==
\begin{figure*}[t]
    \begin{minipage}{0.32\textwidth}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{ l c }
        	   \toprule 
        	   \midrule
        	   \centering
        	   Method & Acc.($\%$)  \\
               \midrule
               Worst Matching & $48.83\%$  \\
               Random Matching & $52.12\%$  \\
               \midrule
               \textbf{Similarity Matching (Ours)} & $\textbf{67.35\%}$  \\
        	   \midrule
        	   \bottomrule
    	   \end{tabular}	
            \label{tbl:analysis_similarity}
        }
    \end{minipage}\hfill
    \begin{minipage}{0.38\textwidth}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{l c c}
        	   \toprule 
        	   \midrule
        	   \centering
        	   Method & IID (P) & NonIID (P) \\
        	   \midrule
        	   FedAvg & $45.99\%$  & $31.43\%$ \\
               FedAvg + Factorization & $49.72\%$ & $34.75\%$ \\
        	  \midrule
        	  \textbf{Factorized-FL (Ours)} & $\textbf{64.21\%}$ & $\textbf{45.37\%}$ \\
        	  \midrule
        	  \bottomrule
        	\end{tabular}	
            \label{tbl:analysis_factorization_2}
        }
    \end{minipage}\hfill
    \begin{minipage}{0.285\textwidth}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{lc}
    	        \toprule 
        	    \midrule
        	    \centering
                Method & Acc.($\%$)  \\
        	    \midrule
        	    \textbf{Factorized-FL (Ours)} & $\textbf{67.35\%}$  \\
                \midrule
                w/o factorization & $63.31\%$  \\
                w/o bias $\mu$ (Only $\textbf{u}$, $\textbf{v}$) & $33.83\%$  \\
                \midrule
        	    \bottomrule
    	    \end{tabular}		
            \label{tbl:analysis_factorization}
        }
    \end{minipage}\hfill
    
    % \vspace{-.45in}
    \\
    \begin{tabular}{ccc}
        \small \hspace{0.15in} (a) Effect of Matching Strategy & 
        \small \hspace{0.85in} (b) Effect of Factorization &
        \small \hspace{0.5in} (c) Ablation Study on Factorization
    \end{tabular}
    
    \\
    \vspace{0.05in}
    \begin{minipage}{0.61\textwidth}
        % \includegraphics[width=0.99\linewidth]{figures/images/sparsity.pdf} 
        \resizebox{0.99\textwidth}{!}{
            \begin{tabular}{ccccccc}
                \toprule 
        	    \midrule
        	    \centering
        	    \multirow{2}{*}{Backbone} & Num. & Num. & Head & Regular & $I \cdot F \times O \cdot F$  & $F \cdot F \times I \cdot O$  \\
        	    & Conv & FC & BN & Kernel & Factorization & Factorization \\
        	    \midrule
        	    \multirow{3}{*}{ResNet-9} & 8 & 1 & - & $61.29\%$ & $60.96\%$ & $\textbf{62.34\%}$ \\
        	    & 8 & 2 & \cmark & $56.08\%$ & $60.81\%$ & $\textbf{62.65\%}$ \\
         	    & 8 & 2 & \xmark & $50.01\%$ & $63.42\%$ & $\textbf{64.39\%}$ \\
         	    \midrule
                \multirow{3}{*}{ResNet-18} & 17 & 1 & - & $63.06\%$ & $55.72\%$ & $\textbf{66.23\%}$ \\
        	    & 17 & 2 & \cmark & $58.36\%$ & $61.39\%$ & $\textbf{68.78\%}$ \\
        	    & 17 & 2 & \xmark  & $51.26\%$ & $63.32\%$ & $\textbf{67.93\%}$ \\
        	    \midrule
        	    \bottomrule 
            \end{tabular}
            \label{tbl:analysis_factorization_3}
        }
    \end{minipage}
    \begin{minipage}{0.38\textwidth}
        \resizebox{0.99\textwidth}{!}{
            \begin{tabular}{ccccc}
                \toprule 
        	    \midrule
        	    \centering
        	    \multirow{2}{*}{Backbone} & \multirow{2}{*}{$\lambda_1$} & Num. & Acc. \\
        	    & & Params. & (\%) \\
        	    \midrule
        	     ResNet-9 & - & 2.574 M (100\%) & $61.95\%$ \\
        	     \midrule
        	     \multirow{5}{*}{\shortstack{Factorized \\ ResNet-9}} &  1e-4 & 2.731 M (106\%) & $63.31\%$ \\
        	      &  3e-4 & 2.515 M (97\%) & $63.74\%$ \\
        	      &  5e-4 & 2.283 M (88\%) & $63.12\%$ \\
        	      &  7e-4 & 2.068 M (80\%) & $62.69\%$ \\
        	      &  1e-3 & 1.784 M (69\%) & $62.67\%$ \\
        	    \midrule
        	    \bottomrule
            \end{tabular}
            \label{tbl:analysis_factorization_4}
        }
    \end{minipage}\hfill
    
    \\
    \begin{tabular}{ccc}
        \small \hspace{0.3in} (d) Analysis of Backbone Network and Factorization Strategy & 
        \small \hspace{0.65in} (e) Analysis of Sparsity Controlled by $\lambda_1$
    \end{tabular}
    
    \vspace{-0.05in}
    \caption{\small \textbf{In-Depth Analysis of Factorized-FL} (a) we show performance depending on different matching strategies, (b) ablation study of our factorization method, (c) impact of factorization method applied to naive federated learning algorithm, (d) analysis of backbone network and factorization strategies, and (e) model size and corresponding accuracy by varying $\lambda_1$. }
    \vspace{-0.2in}
    
    \label{fig:analysis}
\end{figure*}


==> figures/fig_distance.tex <==
\begin{figure*}[t]
\small
\vspace{-0.1in}
    \small
    \centering
    \begin{tabular}{c c c c c c}
        \small    
        \hspace{-0.15in}
        \includegraphics[width=0.155\textwidth]{figures/images/plain_l1_1.png} &
        \hspace{-0.15in} \includegraphics[width=0.155\textwidth]{figures/images/plain_l1_100.png} &
        \hspace{-0.15in} \includegraphics[width=0.155\textwidth]{figures/images/u_l1_1.png} &
        \hspace{-0.15in} \includegraphics[width=0.155\textwidth]{figures/images/u_l1_100.png} &
        \hspace{-0.15in} \includegraphics[width=0.155\textwidth]{figures/images/v_l1_1.png} &
        \hspace{-0.15in} \includegraphics[width=0.155\textwidth]{figures/images/v_l1_100.png} \\
        
        \vspace{-0.05in}
        \hspace{-0.15in}
        
        % \includegraphics[width=0.155\textwidth]{figures/images/plain_l4_1.png} &
        % \hspace{-0.15in} \includegraphics[width=0.155\textwidth]{figures/images/plain_l4_100.png} &
        % \hspace{-0.15in} \includegraphics[width=0.155\textwidth]{figures/images/u_l4_1.png} &
        % \hspace{-0.15in} \includegraphics[width=0.155\textwidth]{figures/images/u_l4_100.png} &
        % \hspace{-0.15in} \includegraphics[width=0.155\textwidth]{figures/images/v_l4_1.png} &
        % \hspace{-0.15in} \includegraphics[width=0.155\textwidth]{figures/images/v_l4_100.png} \\
        
        \includegraphics[width=0.155\textwidth]{figures/images/plain_l8_1.png} &
        \hspace{-0.15in} \includegraphics[width=0.155\textwidth]{figures/images/plain_l8_100.png} &
        \hspace{-0.15in} \includegraphics[width=0.155\textwidth]{figures/images/u_l8_1.png} &
        \hspace{-0.15in} \includegraphics[width=0.155\textwidth]{figures/images/u_l8_100.png} &
        \hspace{-0.15in} \includegraphics[width=0.155\textwidth]{figures/images/v_l8_1.png} &
        \hspace{-0.15in} \includegraphics[width=0.155\textwidth]{figures/images/v_l8_100.png} \\
        
        
        \hspace{-0.1in} $E=1$ &
        \hspace{-0.1in} $E=100$ &
        \hspace{-0.05in} $E=1$ &
        \hspace{-0.05in} $E=100$ &
        \hspace{-0.05in} $E=1$ &
        \hspace{-0.05in} $E=100$ \\
        
        \multicolumn{2}{c}{(a) Regular Kernel } &
        \multicolumn{2}{c}{(b) $\textbf{u}$ of Factorized Kernel}  &
        \multicolumn{2}{c}{(c) $\textbf{v}$ of Factorized Kernel}
        
    \end{tabular}
    \vspace{-0.1in}
    \caption{\small{\textbf{Euclidean Distance of Parameters in Label Heterogeneous Scenario}} Top row indicates the first conv layer and bottom row represents the last conv layer. The brighter color represents the closer the parameters to each other (see Appendix C for full comparison). }
    \label{fig:distance}
    \vspace{-0.1in}
\end{figure*}


==> figures/fig_pfedpara.tex <==
\begin{wrapfigure}[8]{r}{0.45\textwidth}
\centering
\vspace{-0.35in}
\begin{tabular}{cc}
     \includegraphics[width=0.49\linewidth]{figures/images/pfedpara_perf.pdf} &
     \hspace{-0.2in} \includegraphics[width=0.49\linewidth]{figures/images/pfedpara_size.pdf} \\
     (a) Performance & (b) Model Capacity
\end{tabular}
\vspace{-0.1in}
\caption{\textbf{The effect of factorization methods}}
\label{fig:hadamard}
\end{wrapfigure}

==> figures/fig_sparsity.tex <==
\begin{wrapfigure}{r}{8.25cm}
    \includegraphics[\linewidth]{fig}
\end{wrapfigure}

